The bias of dark matter tracers: assessing the accuracy of mapping techniques

We present a comparison between approximated methods for the construction of mock catalogs based on the halo-bias mapping technique. To this end, we use as reference a high resolution $N$-body simulation of 3840$^3$ dark matter particles on a 400$h^{-1}\rm{Mpc}$ cube box from the Multidark suite. In particular, we explore parametric versus non-parametric bias mapping approaches and compare them at reproducing the halo distribution in terms of the two and three point statistics down to $\sim 10^8\,{\rm M}_{\odot}\,h^{-1}$ halo masses. Our findings demonstrate that the parametric approach remains inaccurate even including complex deterministic and stochastic components. On the contrary, the non-parametric one is indistinguishable from the reference $N$-body calculation in the power-spectrum beyond $k=1\,h\,{\rm Mpc}^{-1}$, and in the bispectrum for typical configurations relevant to baryon acoustic oscillation analysis. We conclude, that approaches which extract the full bias information from $N$-body simulations in a non-parametric fashion are ready for the analysis of the new generation of large scale structure surveys.

==> newcomands.tex <==
\newcommand{\eR}{\emph{eROSITA}}
\newcommand{\be}{\begin{equation}}
\newcommand{\dd}{{\rm d}}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\xv}{\textbf{x}}
\newcommand{\dtr}{{\rm d}^{3}r}
\newcommand{\dts}{{\rm d}^{3}s}
\newcommand{\vr}{\textbf{r}}
\newcommand{\vs}{\textbf{s}}
\newcommand{\phzs}{photometric redshifts}
\newcommand{\phz}{photometric redshift}
\newcommand{\hvr}{\hat{\textbf{$\Omega$} }}
\newcommand{\hvs}{\hat{\textbf{s}}}
\newcommand{\hvk}{\hat{\textbf{k}}}
\newcommand{\uv}{\textbf{u}}
\newcommand{\maw}{\mathcal{W}}
\newcommand{\maa}{\mathcal{A}}
\newcommand{\mab}{\mathcal{B}}
\newcommand{\matt}{\mathcal{T}}
\newcommand{\mak}{\mathcal{K}}
\newcommand{\mau}{\mathcal{U}}
\newcommand{\mam}{\mathcal{M}}
\newcommand{\man}{\mathcal{N}}
\newcommand{\mar}{\mathcal{R}}
\newcommand{\magg}{\mathcal{G}}
\newcommand{\tmar}{\tilde{\mathcal{R}}}
\newcommand{\maal}{\mathcal{L}}
\newcommand{\ee}{\end{equation}}
\newcommand{\scr}{\textcolor{red}}
\newcommand{\scg}{\textcolor{green}}
\newcommand{\mav}{\mathcal{V}}
\newcommand{\maf}{\mathcal{F}}
\newcommand{\dtk}{{\rm d}^{3}k}
\newcommand{\dtq}{{\rm d}^{3}q}
\newcommand{\vk}{\textbf{k}}
\newcommand{\yv}{\textbf{y}}
\newcommand{\zv}{\textbf{z}}
\newcommand{\vn}{\textbf{n}}
\newcommand{\vD}{\textbf{D}}
\newcommand{\vp}{\textbf{p}}
\newcommand{\vq}{\textbf{q}}
\newcommand{\vf}{\textbf{f}}
\newcommand{\vell}{{\boldsymbol{\ell}}}
\newcommand{\vdelta}{{\boldsymbol{\delta}}}
\newcommand{\scb}{\textcolor{blue}}
\newcommand{\Omegab}{\mbox{\boldmath$\Omega$}}
\newcommand{\map}{\mathcal{\Pi}}
\newcommand{\mapp}{\mathcal{P}}


\newcommand\mmybox[2][fill=blue!20]{%
    \tikz[baseline]\node[%
        inner ysep=0pt, 
        inner xsep=2pt, 
        anchor=text, 
        rectangle, 
        rounded corners=1mm,
        #1] {\strut#2};%
}

\newcommand\mmyboxout[2][fill=red!20]{%
    \tikz[baseline]\node[%
        inner ysep=0pt, 
        inner xsep=2pt, 
        anchor=text, 
        rectangle, 
        rounded corners=1mm,
        #1] {\strut#2};%
}


\newcommand\mmyboxres[2][fill=blue!40]{%
    \tikz[baseline]\node[%
        inner ysep=0pt, 
        inner xsep=2pt, 
        anchor=text, 
        rectangle, 
        rounded corners=1mm,
        #1] {\strut#2};%
}


\newcommand\mmyboxtitle[2][fill=green!40]{%
    \tikz[baseline]\node[%
        inner ysep=2pt, 
        inner xsep=2pt, 
        anchor=text, 
        rectangle, 
        rounded corners=2mm,
        #1] {\strut#2};%
}

